Get Your Vitamin C! Robust Fact Verification with Contrastive Evidence

Typical fact verification models use retrieved written evidence to verify claims. Evidence sources, however, often change over time as more information is gathered and revised. In order to adapt, models must be sensitive to subtle differences in supporting evidence. We present VitaminC, a benchmark infused with challenging cases that require fact verification models to discern and adjust to slight factual changes. We collect over 100,000 Wikipedia revisions that modify an underlying fact, and leverage these revisions, together with additional synthetically constructed ones, to create a total of over 400,000 claim-evidence pairs. Unlike previous resources, the examples in VitaminC are contrastive, i.e., they contain evidence pairs that are nearly identical in language and content, with the exception that one supports a given claim while the other does not. We show that training using this design increases robustness -- improving accuracy by 10% on adversarial fact verification and 6% on adversarial natural language inference (NLI). Moreover, the structure of VitaminC leads us to define additional tasks for fact-checking resources: tagging relevant words in the evidence for verifying the claim, identifying factual revisions, and providing automatic edits via factually consistent text generation.

==> figures/intro.tex <==
\begin{tikzpicture}
\tikzstyle{bigbox} = [draw=gray!100, thick,  rectangle]
\tikzstyle{box} = [ draw=black,rounded corners,rectangle, fill=gray!30,text width=9cm,align=center]
\tikzstyle{sbox} = [ draw=black,rounded corners,rectangle, fill=gray!30,text width=6cm,align=center]
\tikzstyle{titlebox} = [align=left,text width=10cm]
\tikzstyle{subtitlebox} = []
\tikzstyle{linkbox} = [text=blue]


\node[titlebox] (title) {{\large Beaverton, Oregon}};
\draw[-,draw=gray!100] (title.south west) -- (title.south east);
\node[subtitlebox, below=0.5cm of title.west, anchor=west] (subtitleleft) {{\tiny From Wikipedia, the free encyclopedia}};
\node[subtitlebox, below=0.5cm of title.east, anchor=east] (subtitleright) {{\tiny Revision ID: 336934876}};
% \node[linkbox, below=0.3cm of title.south] (linkboxa) {\underline{\tiny Revision as of 03:58, 12 March 2020}};
\node[box,below= 0.5cm of title.south] (textboxa) {{ its population is estimated to be 86,205, almost 14\% more than the 2000 census figure of 76,129.}};
\node[linkbox, below=0cm of textboxa.south] (linkboxb) {\underline{\tiny Revision as of 04:10, 10 January 2010}};
\node[box,below= 0cm of linkboxb] (textboxb) {{ its population is estimated to be 91,757, almost 14\% more than the 2000 census figure of 76,129.}};

\begin{pgfonlayer}{background}
  \node[bigbox] [fit = (title) (textboxb)] {};
\end{pgfonlayer}
\node[sbox,below of=textboxb] (bottombox) {More than 90K people live in Beaverton};
\node[left=0cm of bottombox.west] (claim) {Claim: };
\draw[->, >=latex, bend right=0, red!70!yellow, line width=10pt] (-4.6,-1.4)  to node[white,sloped]{\bf Refutes{\quad}{\quad\quad\quad}} ([xshift=0.1cm,yshift=0.1cm]bottombox.west);
\draw[->, >=latex, bend right=0, green!70!red, line width=10pt] (4.6,-2.5) to node[white,sloped,]{\quad \bf Supports} ([xshift=-0.1cm]bottombox.east);
\end{tikzpicture}

==> figures/intro_old.tex <==
\begin{tikzpicture}
\tikzstyle{bigbox} = [draw=gray!100, thick,  rectangle]
\tikzstyle{box} = [ draw=black,rounded corners,rectangle, fill=gray!50,text width=10cm,align=center]
\tikzstyle{sbox} = [ draw=black,rounded corners,rectangle, fill=gray!50,text width=5cm,align=center]
\tikzstyle{titlebox} = [align=left,text width=10cm]
\tikzstyle{subtitlebox} = []
\tikzstyle{linkbox} = [text=blue]


\node[titlebox] (title) {{\large Severe acute respiratory syndrome coronavirus 2}};
\draw[-,draw=gray!100] (title.south west) -- (title.south east);
\node[subtitlebox, below=0.5cm of title.west, anchor=west] (subtitleleft) {{\tiny From Wikipedia, the free encyclopedia}};
\node[subtitlebox, below=0.5cm of title.east, anchor=east] (subtitleright) {{\tiny Revision ID: 945154642}};
\node[linkbox, below=0.3cm of title.south] (linkboxa) {\underline{\tiny Revision as of 03:58, 12 March 2020}};
\node[box,below= 0cm of linkboxa] (textboxa) {{ On 30 January 2020, SARS-CoV-2 was designated a Public Health\\ Emergency of International Concern by the WHO.}};
\node[linkbox, below=0cm of textboxa.south] (linkboxb) {\underline{\tiny Revision as of 04:02, 12 March 2020}};
\node[box,below= 0cm of linkboxb] (textboxb) {{ On 30 January 2020, SARS-CoV-2 [$\dots$] by the WHO, {\bf and on 11}\\{\bf     \quad March 2020 the WHO declared it a pandemic.}}};

\begin{pgfonlayer}{background}
  \node[bigbox] [fit = (title) (textboxb)] {};
\end{pgfonlayer}
\node[sbox,below of=textboxb] (bottombox) {COVID-19 is a global pandemic};
\node[left=0cm of bottombox.west] (claim) {Claim: };
\draw[->, >=latex, bend right=20, red!70!yellow, line width=10pt] (-5,-1.5)  to node[white,rotate=-51,yshift=-0.4ex]{\bf Refutes{\quad\quad}{\quad\quad\quad}} ([xshift=0.1cm,yshift=0.1cm]bottombox.west);
\draw[->, >=latex, bend right=0, green!70!red, line width=10pt] (4.7,-3) to node[white,sloped,]{\quad \bf Supports} ([xshift=-0.1cm]bottombox.east);
\end{tikzpicture}

==> sections/ethical.tex <==
\section*{Ethical Considerations}
This work aims to provide a resource for furthering research and development on tasks relating to fact verification. Fact verification, and its surrounding ecosystem, is a sensitive and delicate subject---especially in the face of the mis- and disinformation that is widespread today. Automated fact checking systems are promising tools for stymying this modern phenomenon---and hence, improving their robustness and reliability is a critical and impactful consideration. Of course, the dataset and models presented in this work do not, and should not, serve as standalone solutions. Though automated systems such as the ones developed in this paper may very well aide in slowing the spread of fake news, their use alone does not absolve any moderating parties of their possible responsibilities to employ additional measures for stronger oversight.

In terms of the data collection practices of this work, we based \thedataset off of Wikipedia, a free and open resource. During the creation of \thedataset, we sourced and paid annotators via a fixed-sum contract with TransPerfect. The general terms and conditions of our contract included standard provisions ensuring fair worker treatment---such as equal employment opportunity and affirmative action, federal labor law regulations, and overtime compensation requirements.
TransPerfect followed a quality assurance procedure in which a group of experts reviewed all annotations. In addition, the data was delivered in batches and we reviewed a random set of examples each time, provided feedback, and asked for corrections if needed.

==> sections/models.tex <==
\section{Modeling} \label{sec:models}
\regina{merge with 4?}
\regina{give examples all over...}
In this section we describe the baseline models we evaluate on the various \thedataset tasks.

\subsection{Factual Revision Flagging.} 

% \begin{itemize}[leftmargin=*]
    \tpf{Edit Distance.} We measure the Levenshtein distance between $s_{t-1}$ and $s_t$, assuming that larger edits are more likely to represent substantive changes. We tune a decision threshold on the training set.
    
    \paragraph{BOW.} We use an MLP on top of a bag-of-words representation. Each sentence is encoded as $e_*$, the average  \emph{fast}Text~\citep{bojanowski-etal-2017-enriching} word embedding of its edited words (i.e., that were removed or modified in the revision). The MLP input is then taken as $[e_{t-1}; e_{t};|e_{t} - e_{t-1}|; e_{t} \cdot e_{t-1}].$
    
    \paragraph{ALBERT.} We train the ALBERT transformer~\cite{lan-etal-2020-learning} using either only the edited words (diff), or the full sentence pair (full).
    
    % \item ALBERT (diff): an ALBEBRT-base~\citep{ALBERT2020} transformer classifier on top of the edited words of each sentence.
    
    % \item ALBERT (full): an ALBEBRT-base model classifier on top of the two full sentences $\revtup$.
% \end{itemize}


\subsection{Contextual Fact Verification}
\label{sec:fact-model}
We train an ALBERT sentence-pair classifier to predict $\rel(c,s)$. Compared to BERT~\citep{devlin-etal-2019-bert}, it uses fewer parameters by shrinking the embedding size and sharing layers, which we find improves the robustness of fact verification models.
% \tal{todo}

\subsection{Word-level Rationales}

\tpf{Unsupervised.} As in \citet{shah2020automatic}, we optimize a Lagrangian relaxation of Eq.~\ref{eq:rationale}, where
\[
\mathcal{L}_{\mathrm{us}} := -\log p(\rel(c, s \odot m) = \NEI) + \frac{\lambda}{n} \sum_{i=1}^n m_i.
\]

We keep the sentence-pair classifier $\rel$ (from \S\ref{sec:fact-model}) fixed, and train a separate ALBERT model to predict the mask $m$ using a Gumbel softmax.

\paragraph{Distantly supervised.} By leveraging opposing claims present in \thedataset, we are able to identify $m_{\mathrm{edit}} = \texttt{diff}(s_{t-1}, s_t)$---i.e., the non-stopwords that are deleted or replaced in $s_{t-1}$ when compared to $s_t$. We then use $m_{\mathrm{edit}}$ as distant supervision for $m$, where
$\mathcal{L}_{\mathrm{ds}} = -\frac{\gamma}{n}\sum_{i=1}^n \log p(m_i = m_{\mathrm{edit}_i})$. We combine both the $\mathcal{L}_{\mathrm{us}}$ and $\mathcal{L}_{\mathrm{ds}}$ losses.

\subsection{Factually Consistent Generation}
We use the BART-base  sequence-to-sequence transformer-based generator~\citep{lewis-etal-2020-bart}. BART was pre-trained to reconstruct sentences from their noisy versions, arguably filling missing information to be consistent with the rest of the text. We fine-tune it on our generation tasks. We concatenate the two input sentences with a special separator as input, and provide the desired output sentence for the decoder.

==> tables/res_nli.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lrrr|rrr}
\toprule
Train dataset & VitD real & VitD syn & MNLI  & ANLI-1 & ANLI-2  & ANLI-3 \\
\midrule
MNLI                & 44.93 &	69.67 &	85.22 &	31.30 &	28.00 &	32.25 \\
VitD                 & 86.16 &	89.78 &	69.18 &	\textbf{41.60} &	\textbf{34.50} &	\textbf{35.92}             \\
VitD + MNLI         & 86.68 &	91.18 &	85.95 &	38.20 &	33.60 &	31.67 \\
\bottomrule
\end{tabular}

\caption{\thedataset improves the robustness of NLI classifiers.} \label{tab:res_fact_ver}

\end{table*}
